Patrol Security Game: Defending Against Adversary with Freedom in Attack Timing, Location, and Duration

We explored the Patrol Security Game (PSG), a robotic patrolling problem modeled as an extensive-form Stackelberg game, where the attacker determines the timing, location, and duration of their attack. Our objective is to devise a patrolling schedule with an infinite time horizon that minimizes the attacker's payoff. We demonstrated that PSG can be transformed into a combinatorial minimax problem with a closed-form objective function. By constraining the defender's strategy to a time-homogeneous first-order Markov chain (i.e., the patroller's next move depends solely on their current location), we proved that the optimal solution in cases of zero penalty involves either minimizing the expected hitting time or return time, depending on the attacker model, and that these solutions can be computed efficiently. Additionally, we observed that increasing the randomness in the patrol schedule reduces the attacker's expected payoff in high-penalty cases. However, the minimax problem becomes non-convex in other scenarios. To address this, we formulated a bi-criteria optimization problem incorporating two objectives: expected maximum reward and entropy. We proposed three graph-based algorithms and one deep reinforcement learning model, designed to efficiently balance the trade-off between these two objectives. Notably, the third algorithm can identify the optimal deterministic patrol schedule, though its runtime grows exponentially with the number of patrol spots. Experimental results validate the effectiveness and scalability of our solutions, demonstrating that our approaches outperform state-of-the-art baselines on both synthetic and real-world crime datasets.

==> unused/evaluation_ting.tex <==
\begin{figure}
	\centering
	\includegraphics[width=.7\linewidth]{new_fig/EMRvsR.pdf}
	\caption{The values of expected maximum reward (EMR) and Entropy rate when the input parameter $\alpha=(1,4,7,9)$. TSP-b has the most efficient tradeoff since it achieves the lowest EMR with the highest entropy rate.}
	\label{fig:two_criteria}
	
\end{figure}


%simulation for table
%\begin{table*}[]
%    \begin{tabular}{c|l|l|l|l|l|l|l|l|l|l}
%        \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Constant\\ RP: 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Linear\\ RP:0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Quadratic\\ RP: 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Linear\\ RP:.6\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Linear\\ RP:1.2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}M2\\ Linear, RP: .6\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}M3\\ Linear, RP: .6\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}M1\\ Denver\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}M2\\ Denver\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}M3\\ Denver\end{tabular}} \\ \hline
%        RS                    & 1.00 (.000)                                                                   & .549 (.000)                                                                & .694 (.187)                                                                    & .037 (.001)                                                                 & .001 (.000)                                                                  & .127 (.007)                                                                      & .065 (.008)                                                                      & \textbf{1.00}                                                            & \textbf{.809}                                                            & \textbf{.877}                                                           \\ \hline
%        AF                    & 1.04 (.001)                                                                   & \textbf{.029 (.001)}                                                       & \textbf{.010 (.000)}                                                           & .012 (.000)                                                                 & .012 (.000)                                                                  & .017 (.000)                                                                      & .000                                                                             & 2.19                                                                     & 5.76                                                                     & .988                                                                    \\ \hline
%        SG                    & 1.35 (.008)                                                                   & .057 (.004)                                                                & .062 (.007)                                                                    & \textbf{.001 (.000)}                                                        & \textbf{.000 (.000)}                                                         & .000 (.000)                                                                      & .000                                                                             & 1.11                                                                     & 4.21                                                                     & 5.69                                                                    \\ \hline
%        maxEn                 & 1.32 (.017)                                                                   & 1.52                                                                       & 7.03 (53.1)                                                                    & 1.01                                                                        & .289                                                                         & 1.31                                                                             & .6                                                                               & 3.31                                                                     & 6.11                                                                     & 9.97                                                                    \\ \hline
%        minKC                 & 1.14 (.001)                                                                   & 0.61                                                                       & 2.60 (9.54)                                                                    & .076                                                                        & .002                                                                         & 6.76                                                                             & 1.7                                                                              & 1.53                                                                     & 5.99                                                                     & 7.52                                                                   
%    \end{tabular}
%\end{table*}

%simulation 
%
%\begin{table*}[ht]
%    \small
%    \captionsetup{justification=justified,singlelinecheck=false}
%    \begin{center}
%        \begin{tabular}{|c| c c c c|}
%            \hline
%            & Constant, $RP$=0 & Linear, $RP$=0 & Linear, $RP$=1.2 & Denver \\ \hline
%            M1              
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_0_model_m1_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m1_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m1_penalty_3_.pdf}
%            \end{minipage}
%            
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/denver_h_1_model_m1_.pdf}
%            \end{minipage}
%            
%            \\ \hline 
%            M2              
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_0_model_m2_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m2_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m2_penalty_3_.pdf}
%            \end{minipage}
%            
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/denver_h_1_model_m2_.pdf}
%            \end{minipage}
%            \\ \hline 
%            M3              
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_0_model_m3_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m3_penalty_1_.pdf}
%            \end{minipage}
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/payoff_differ_h_1_model_m3_penalty_3_.pdf}
%            \end{minipage}
%            
%            & \begin{minipage}{.45\columnwidth}
%                \centering
%                \includegraphics[width=.94\linewidth]{fig/denver_h_1_model_m3_.pdf}
%            \end{minipage}            
%            \\ \hline
%        \end{tabular}        
%        \caption{\label{table:main_results} \rey{R2: M is overloaded} Each row represents an attacker model (M1: full visibility, M2: local visibility, M3: no visibility) and each column represents a specific setup. In each figure, the $y$-axis is the relative attacker's payoff (the lower the value, the better the performance of the patrol route) and each bar represents a solution, which is TSP-b (T), Bwalk (B), SG (S), minimum Kemeny constant (minKC), or maximum entropy (maxEn). Generally, Bwalk performs well in low RP cases, SG performs well in linear utility functions, and TSP-b has low attacker's payoff among all cases. }  
%    \end{center}
%\end{table*}


\section{Experiments}
We evaluate the proposed algorithms, \textit{TSP-based} (TSP-b), \textit{Biased random walk} (Bwalk), and \textit{State graph walk} (SG), with two baselines \textit{Markov chains with minimal Kemeny constant} (minKC)~\cite{patel2015robotic} and \textit{Markov chains with maximum entropy} (maxEn)~\cite{george2018markov}. The experiments are based on artificial datasets and Denver crime dataset~\cite{city2016denver} with three different attacker models, Full visibility (Full vis.), Local visibility (Local vis.), and No visibility (No vis.). There are three major observations.
\begin{enumerate}
	\item Our algorithms realize the tradeoff between expected maximum reward (EMR) and entropy rate. For comparison, TSP-b and Bwalk have more freedom to control EMR and entropy rate with parameter $\alpha$ (Figure~\ref{fig:two_criteria}).
	
	\item For all algorithms, when the penalty increased, the attacker's (expected) payoff decreased. For the same evaluation setup, the attacker's payoff is the minimum when the attacker adopts the model of no visibility, and the highest, when the attacker adopts full visibility. Roughly speaking, MaxEn performs worse than our algorithms among all setups. TSP-b, Bwalk, and SG performs well when the utility function is not constant (Figure~\ref{fig:linear_md1},~\ref{fig:quad_md1}). MinKC has comparable performance when the utility function is constant. In addition, our algorithms have low standard errors in all settings (Table~\ref{table:main_results}).
	
	\item TSP-b and Bwalk are more scalable with the increase in the number of spots. One reason is that these algorithms are perturbed the tours from TSP/BGT, which are more delicate designed routes (Figure~\ref{fig:scalability}).  
\end{enumerate}


We define a unit length as the distance that the patroller takes a one-time slot to travel. For simulations, all spots are randomly generated from a $20000 \times 20000$ grid. Without specification, the number of spots in a setup is 30. For Denver dataset, the geographic range is in Denver City only, which has 78 neighborhoods. We set up the utility functions as polynomial ones with maximum degrees 0 (constant) or 1 (linear) for demonstration. Each one represents a different type of crimes. The coefficients of utility functions are generated uniform randomly between $.001$ to $1$. In the real-world setting, we use the Denver Crime Dataset to learn the coefficient based on the number of crimes among different types in each neighborhood. For the baselines, minKC, and maxEn subject to stationary distribution constraints. To fit the setup of utility functions, we set up the stationary distribution for each spot $j$ propositional to $b_j$, where $b_j$ is the coefficient of the maximum degree in its utility function $h_j$.

    In the game, each solution generates a patrol schedule as the defender's strategy. The attacker's payoff $Z$ is realized by attacking spot $i$ from time $t_s$ to $t_e$. In this setting, we empirically calculated the expected payoff to all possible spot $i$ according to all possible attack period $t_s, t_e$ under specific attacker models. We then derived the attacker's maximum (expected) payoff. Due to the raw values are high, all payoff values are divided by $\zeta^{d+1}$, where $\zeta$ is the diameter of all spots.
%we use the attacker's maximum payoff of the schedules generated by BGT (introduced in Section~\ref{alg:BGT explanation}) as the baseline, which we denote by \emph{Attacker relative payoff}. That is, the (maximum) payoff of BGT set to 1 and the others are divided by the payoff of BGT. It is because BGT provides deterministic schedules, which makes the attacker's maximum payoff consistent compared with other algorithms. 
In each experiment, each bi-criteria algorithm generates around 8 to 10 schedules based on different values of parameter $\alpha$. The values of $\alpha$ are uniformly generated in the following domains. TSP-b: $[0.1,1]$, Bwalk: $[0,4.5]$, SG: $[0,80]$. Generally speaking, increasing the number of $\alpha$ values would increase the performance of the algorithm but takes more computation time, which is a performance-complexity trade-off.

%In each experiment, we ran 50 trials to get the average and standard error of the maximum payoff for each algorithm.

\subsection{EMR v.s. entropy rate}
Figure~\ref{fig:two_criteria} reports the performance of algorithms under \emph{expected maximum reward} and \emph{entropy rate}, which are mentioned in Section~\ref{sec:general_cases_algo}. In y-axis, we scale the EMR as 1 if the maximum reward is generated by BGT. Each point represents the schedule which is generated by different algorithms and the digit aside each point denotes the value of the input parameter $\alpha$. $\alpha$ is unified from 1 to 10 among three proposed algorithms, where the real-value may from different domains. For example, in TSP-b, the skip probability is 0 as $\alpha=1$ and the skip probability is $90\%$ as $\alpha=10$. For TSP-b and Bwalk, the higher the value of $\alpha$ indicates the higher randomness of the schedule. For SG, the lower the value of $\alpha$ indicates the higher randomness of the schedule. In fact, one can see that the entropy rate and EMR increased with higher $\alpha$ value in TSP-b and Bwalk. However, this tradeoff is not that clear in SG for a high $\alpha$ value. 
%Generally, TSP-b has the most efficient tradeoff since it can achieve low EMR with high entropy rate.



%simulation for table
\begin{table*}[]
	\captionsetup{justification=centering,singlelinecheck=false}
	\begin{tabular}{llll}
		\multicolumn{3}{c}{
			\centering
			\includegraphics[width=.43\linewidth]{Figures/legend_plot.png}
			
		} \\
		%row 0        
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}                        
			\includegraphics[width=.94\linewidth]{Figures/polyd1_m1_random.pdf}
			\vspace{-4mm}
			\captionof{figure}{Constant utility, Full vis.}\label{fig:constant_md1}
		\end{minipage}  & 
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}            
			\includegraphics[width=.94\linewidth]{Figures/polyd2_m1_random.pdf}
			\vspace{-4mm}
			\captionof{figure}{Linear utility, Full vis.}\label{fig:linear_md1}
		\end{minipage}     & 
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}            
			\includegraphics[width=.94\linewidth]{Figures/polyd3_m1_random.pdf}
			\vspace{-4mm}
			\captionof{figure}{Quadratic utility, Full vis.}\label{fig:quad_md1}
		\end{minipage} &  \\
		
		%row 1
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}            
			\includegraphics[width=.94\linewidth]{Figures/polyd1_m2_random.pdf}
			\vspace{-4mm}
			\captionof{figure}{Constant utility, Local vis.}\label{fig:constant_md2}
		\end{minipage}  & 
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}            
			\includegraphics[width=.94\linewidth]{Figures/polyd1_m3_random.pdf}
			\vspace{-4mm}
			\captionof{figure}{Constant utility, No vis.}\label{fig:constant_md3}
		\end{minipage}     & 
		
		\begin{minipage}{.65\columnwidth}
			\centering
			\vspace{2mm}            
			\includegraphics[width=.94\linewidth]{Figures/denver_poly_2.pdf}
			\vspace{-4mm}
			\captionof{figure}{Denver, Full vis.}\label{fig:Denver_md1}
		\end{minipage} & 
	\end{tabular}
	\vspace{1mm}
	\caption{Comparing attacker's expected payoff (the lower the value, the better the performance of the patrol route) of our algorithms (TSP-b, Bwalk, SG) and baselines (minKC, maxEN) with different settings and attacker models. Figure~\ref{fig:constant_md1},~\ref{fig:constant_md2},~\ref{fig:constant_md3} are constant utility functions under Full visibility, Local visibility, and No visibility. Figure~\ref{fig:linear_md1},~\ref{fig:quad_md1} are linear and quadratic utility functions under Full visibility. Figure~\ref{fig:Denver_md1} is the simulation on Denver Crime Dataset with full visibility.}    \label{table:main_results}
	
\end{table*}


\vspace{-1mm}
\subsection{Attacker's payoff in artificial and real-world scenario}

The experiments are examined with the following variables; penalty values, the maximum degree of utility functions (1, 2, 3), and the attacker models (Full vis., Local vis., No vis.). The last figure reports the simulation result of Denver crime dataset.

Each figure shows the attacker's (expected) payoff under different penalties. Each realization has been run 10 times and the y-axis is the average attacker's payoff with standard errors. We interpret an algorithm has better performance if and only if the attacker has the lower payoff in the schedule generated by this algorithm.

In the experiments of constant utility functions (Figure~\ref{fig:constant_md1},~\ref{fig:constant_md2},~\ref{fig:constant_md3}), one can see that the payoff drop down when the penalty increased. In addition, attackers with lower visibility (E.g., Full visibility v.s. No visibility) also has a lower payoff. Although TSP-b performs the best in Full vis., minKC is comparable in Local and No vis.. This reflects our observation in Section 4.2 and 4.3, that the optimal solution has a strong correlation with the minimum hitting time.

In the experiments of non-constant utility functions (Figure~\ref{fig:linear_md1},~\ref{fig:quad_md1},~\ref{fig:Denver_md1}), our algorithms clearly outperform the baselines in most cases. For example, the attacker's payoff is 344 for minKC but only 0.46 for SG in the case of linear utility functions, 600 penalty value. One possible reason is that minKC and maxEn are designed only for linear vertex weight and they are not suitable for non-constant utility functions. On the other hand, our algorithms focus on the two objectives: EMR and entropy rate, which are not limited to the degree of utility functions.

%Each row represents an attacker model, where M1 is full visibility, M2 is local visibility, M3 is no visibility. Each cell in the table corresponds to a figure of evaluation among all algorithms. 
%The $y$-axis is \emph{Attacker relative payoff}. That is, the payoff of the schedule is divided by the payoff of BGT. Each bar represents a solution, which is TSP-b (T), Bwalk (B), SG (S), minimum Kemeny constant (minKC), or maximum entropy (maxEn). We interpret an algorithm has better performance if and only if the attacker has the lower \emph{Attacker relative payoff} in the schedule generated by this algorithm.

%In the experiment of constant utility functions with zero penalty (column 1), the attacker's payoff does not change much among all algorithms. minKC performs the best in most attacker models, which reflects the previous discussion that the optimal solution has a strong correlation with minimum hitting time in this special configuration. When utility functions are linear (column 2 and 3), the proposed algorithms are much adaptive compared with minKC and maxEn. E.g., Attacker can collect 10000 times more payoff in minKC comparing with Bwalk in M3, zero penalty and 2000 times more comparing with SG in M1, 1.2 penalties. 

%maxEn has better performance when penalties increased, though it is not clear in this Table. In fact, when we set up the penalties as 4.5 relative payoffs the attacker expected payoff goes down 0.5, which showed that a schedule with high entropy is more adaptive in scenarios with high penalties.

%In Denver crime dataset (column 4), we use the records of burglary crimes between years from 2011 to 2016 and assume the defender patrols between the center of each neighborhood, which is defined as the midpoint of geolocations where the crimes happened in that neighborhood. The weight of each neighborhood is learned by the crime rate. I.e., the weight of a neighbor $i$ is the number of crimes in $i$ divided by the total number of crimes. 1 slot of time is defined as the time of the patroller moving in one meter. The result shows that TSP-b has lowest attacker's payoff in most cases. 

\begin{figure}
	\centering
	\includegraphics[width=.85\linewidth]{Figures/scale.png}
	
	\caption{The attacker relative payoff when the number of spots increased. TSP-b and Bwalk show better and stable performance in high scale scenario.}
	\label{fig:scalability}
	
\end{figure}


\subsection{Scalability}
Figure~\ref{fig:scalability} reports the scalability of the solutions. The settings are full visibility attacker model, constant utility functions, and 0 penalty value for demonstration. To compare the performance under different setups, all attacker's expected payoff is divided by the payoff of BGT patrol route. When the number of spots is more than 100, the solution of minKC is incalculable in our machine due to memory constraint (the solution minKC is calculated by CXYOPT in a laptop of Intel i7-4700 MQ 240GHz CPU with 32 GB ram). 

For other solutions, the 3 proposed algorithms have better performance than maxEn. Comparing within the proposed algorithms, SG has the worst performance. One reason is that schedules generated by SG have higher randomness. When the number of spots increasing which make the topology becomes complicated, it requires a schedule with more delicate designed routes. Thus, TSP-b and Bwalk perform better since their schedules are perturbed from TSP/BGT tours.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%老師看底下那些圖是要留的我再改成現在的格式，fig:scalability 150和300個點還沒跑完，跑完我再改圖
\section{Scalability}
Figure~\ref{fig:scalability} reports the scalability of the solutions. We use the same setting as ~\ref{fig:two_criteria} but with different size of graph. To compare the performance under different setups, all attacker's expected payoff is divided by the payoff of BGT patrol route. When the number of spots is more than 100, the solution of minKC is incalculable in our machine due to memory constraint. MaxEn performs worse than other strategies in scenarios with large graph sizes. For instance, its performance is 100 times worse than SG in cases with 100 spots and 10 times worse in cases with 200 spots. To ensure a clearer comparison and display, we will not include these results in the chart. 

Comparing within the proposed algorithms, SG has the worst performance. One reason is that schedules generated by SG have higher randomness. When the number of spots increasing which make the topology becomes complicated, it requires a schedule with more delicate designed routes. 

It's worth mentioning that the efficiency of Bwalk and the selection of $\alpha$ are influenced by the structure of the graph. In equation~\ref{bwalk}, when a spot $i$ is considerably far from other points, the probability of reaching spot $i$ within the stochastic matrix $P'$ is significantly reduced. This effect is further more as the value of $\alpha$ increases. This scenario leads to the algorithm requiring more time to find a tour that visits all spots.

\section{GPN-based Strategy}
From our experiments, we observed that adjusting the BGT weight order only improves performance in settings with constant utility functions in generalize case, compared to scenarios without any modifications (fig.~\ref{fig:gpn-base_comparison}). One possible reason is that careful adjustment of the tour based on weight is particularly critical, especially with high-degree utility functions. In our experiments, we also compared TSP-b scenarios with and without additional adjustments to the skipping probabilities(fig.~\ref{fig:tsp-base_comparison}). In these comparative experiments, it show that although methods with additional adjustments can achieve lower payoffs, as the degree of the utility function increases, obtaining similarly low payoffs requires higher penalties compared to scenarios without adjustments.  We observe that increasing randomness by reasonably skipping nodes might significantly impact the performance in high penalties case. However, GPN performs well in settings with low penalties and high-degree utility functions. Moreover, GPN exhibits the stable and well performance in terms of scalability, underscoring the potential of this method.

\begin{figure}
\centering
\subfigure[Constant utility, Full vis. ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d1.png}}
\hfill
\subfigure[Linear utility, Full vis]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d2.png}}
\hfill
\subfigure[Quadratic utility, Full vis ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d3.png}}
\hfill
\caption{The full visibility in group-balanced case}
\label{fig:groupadjust_fullvis} %% label for entire figure
\end{figure}

\begin{figure}
\centering
\subfigure[Constant utility, local vis. ]{
\includegraphics[width=0.9\linewidth]{Figures/m2_d1.png}}
\hfill
\subfigure[Constant utility, No vis.]{
\includegraphics[width=0.9\linewidth]{Figures/m3_d1.png}}
\hfill
\caption{The local visibility case and no visibility in group-balanced case}
\label{fig:groupadjust_noandlocal} %% label for entire figure
\end{figure}

\begin{figure}
\centering
\subfigure[Constant utility, Full vis. ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d1_general.png}}
\hfill
\subfigure[Linear utility, Full vis]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d2_general.png}}
\hfill
\subfigure[Quadratic utility, Full vis ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d3_general.png}}
\hfill
\caption{The full visibility case in general case}
\label{fig:general} %% label for entire figure
\end{figure}

\begin{figure}
\centering
\subfigure[Constant utility, Full vis. ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d1_skip_comp.png}}
\hfill
\subfigure[Linear utility, Full vis]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d2_skip_comp.png}}
\hfill
\caption{The comparison of TSP-b and TSP-b-a in general case}
\label{fig:tsp-base_comparison} %% label for entire figure
\end{figure}

\begin{figure}
\centering
\subfigure[Constant utility, Full vis. ]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d1_gpn_comp.png}}
\hfill
\subfigure[Quadratic utility, Full vis]{
\includegraphics[width=0.9\linewidth]{Figures/m1_d3_gpn_comp.png}}
\hfill
\caption{The comparison of GPN and GPN-a in general case}
\label{fig:gpn-base_comparison} %% label for entire figure
\end{figure}


==> unused/probdef.tex <==
% H entropy. S schedule. v_i point of interest. j point in the schedule.


\section{Problem Definition}
There is a weighted complete graph $G=(V,E)$ to represent the points of interest and the distance between any two points. For convince, the edge weight is the number of time slots the patroller needs to travel between. In addition, each vertex might also have a weight to represent the importance of that point. The output would be a schedule which is an infinity long list. Each element in the list is a point $v_i \in V$ and the patroller visits nodes according to the order of the list. We also define the darkness length as the period of time between two consecutive visits on a point to measure the performance of a schedule. In this research, we aim to minimize the maximum of darkness among all points to provide good performance bounds in our designed schedules. For your information, in this paper, we may also use the term ``window size'' to represent the term ``maximum darkness length among all points.''

On the other hand, to model the ability of the adversary, we assume the adversary cannot know the whole schedule but he can fully observe the historical data that patroller already visited and well predict the patroller's next visit if he observes certain patterns of the historical data. Under these constraints, we use Shannon entropy \cite{shannon_entropy2001} from information science to measure the prediction factor for a schedule. For a non-deterministic schedule, each element $j$ in the schedule is a random variable $X_j$ that follows some probability distribution. Therefore we can calculate the entropy $H$ of each element $X_j$ as the following:
\begin{displaymath}
H(X_j)=\sum_{i=1}^{n} P(x_i)\ln \frac{1}{P(x_i)},
\end{displaymath}
where $\{x_1,x_2,,,x_n\}$ are the possible values of $X_j$. Furthermore, the entropy of a schedule $S$ can be calculated as the following:

\begin{displaymath}
H(S)=\lim_{m\to\infty} \frac{\sum_{j=1}^{m}H(j)}{m}=E[H(X)].
\end{displaymath}

Here, the entropy of a schedule can be treated as the expected increase entropy of each element.


Generally speaking, to simultaneously guarantee the patrol performance but also lower the prediction factor for the security reasons, we focus on this bi-criteria problem: how to design a nondeterministic schedule such that the maximum darkness among all points is minimized and the entropy is maximized.
